Normalizing Weak Boson Pair Production at the Large Hadron Collider

The production of two weak bosons at the Large Hadron Collider will be one of the most important sources of SM backgrounds for final states with multiple leptons. In this paper we consider several quantities that can help normalize the production of weak boson pairs. Ratios of inclusive cross-sections for production of two weak bosons and Drell-Yan are investigated and the corresponding theoretical errors are evaluated. The possibility of predicting the jet veto survival probability of VV production from Drell-Yan data is also considered. Overall, the theoretical errors on all quantities remain less than 5-20%. The dependence of these quantities on the center of mass energy of the proton-proton collision is also studied.

==> differences <==
1c1
< \begin{thebibliography}{74}
---
> \begin{thebibliography}{70}
16,18c16,18
< \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Collaboration}},
<   \emph{\bibinfo{title}{Cms ptdr v.2: Physics performance}},
<   \bibinfo{howpublished}{CERN/LHCC 2006-021}.
---
> \bibinfo{author}{\bibfnamefont{CMS}~\bibnamefont{Collaboration}},
>   \emph{\bibinfo{title}{CMS PTDR V.2: Physics Performance}},
>   \bibinfo{howpublished}{CERN/LHCC 2006-021 (2006)}.
21,23c21,23
< \bibinfo{author}{\bibfnamefont{T.~A.} \bibnamefont{Collaboration}},
<   \emph{\bibinfo{title}{Detector and physics performance technical design
<   report}}, \bibinfo{howpublished}{CERN-LHCC/99-14/15 (1999)}.
---
> \bibinfo{author}{\bibfnamefont{ATLAS} \bibnamefont{Collaboration}},
>   \emph{\bibinfo{title}{Detector and Physics Performance Technical Design
>   Report}}, \bibinfo{howpublished}{CERN-LHCC/99-14/15 (1999)}.
92,96d91
< \bibitem[{\citenamefont{Grazzini}(2008)}]{Grazzini:2008tf}
< \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Grazzini}},
<   \bibinfo{journal}{JHEP} \textbf{\bibinfo{volume}{02}}, \bibinfo{pages}{043}
<   (\bibinfo{year}{2008}), \eprint{0801.3232}.
< 
228a224
> 
230c226
< \bibinfo{author}{\bibfnamefont{I.~A.} \bibnamefont{{\it et al.}}},
---
> \bibinfo{author}{\bibfnamefont{I.~Agapov} \bibnamefont{{ et~al.}}},
236c232
< \bibinfo{author}{\bibfnamefont{J.~P.} \bibnamefont{{\it et al.}}},
---
> \bibinfo{author}{\bibfnamefont{J.} \bibnamefont{Pumplin {\it et al.}}},
316,348d311
< \bibitem[{\citenamefont{Ladinsky and Yuan}(1994)}]{Ladinsky:1993zn}
< \bibinfo{author}{\bibfnamefont{G.~A.} \bibnamefont{Ladinsky}} \bibnamefont{and}
<   \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
<   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D50}},
<   \bibinfo{pages}{4239} (\bibinfo{year}{1994}), \eprint{hep-ph/9311341}.
< 
< \bibitem[{\citenamefont{Balazs and Yuan}(1997)}]{Balazs:1997xd}
< \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Balazs}} \bibnamefont{and}
<   \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
<   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D56}},
<   \bibinfo{pages}{5558} (\bibinfo{year}{1997}), \eprint{hep-ph/9704258}.
< 
< \bibitem[{\citenamefont{Landry et~al.}(2003)\citenamefont{Landry, Brock,
<   Nadolsky, and Yuan}}]{Landry:2002ix}
< \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Landry}},
<   \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Brock}},
<   \bibinfo{author}{\bibfnamefont{P.~M.} \bibnamefont{Nadolsky}},
<   \bibnamefont{and} \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
<   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D67}},
<   \bibinfo{pages}{073016} (\bibinfo{year}{2003}), \eprint{hep-ph/0212159}.
< 
< \bibitem[{\citenamefont{Balazs and Yuan}(1999)}]{Balazs:1998bm}
< \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Balazs}} \bibnamefont{and}
<   \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
<   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D59}},
<   \bibinfo{pages}{114007} (\bibinfo{year}{1999}), \eprint{hep-ph/9810319}.
< 
< \bibitem[{\citenamefont{Frederix and Grazzini}(2008)}]{Frederix:2008vb}
< \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Frederix}} \bibnamefont{and}
<   \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Grazzini}},
<   \bibinfo{journal}{Phys. Lett.} \textbf{\bibinfo{volume}{B662}},
<   \bibinfo{pages}{353} (\bibinfo{year}{2008}), \eprint{0801.2229}.
< 
384,388d346
< \bibitem[{\citenamefont{Grazzini}(2006)}]{Grazzini:2005vw}
< \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Grazzini}},
<   \bibinfo{journal}{JHEP} \textbf{\bibinfo{volume}{01}}, \bibinfo{pages}{095}
<   (\bibinfo{year}{2006}), \eprint{hep-ph/0510337}.
< 
481,489d438
< \bibitem[{\citenamefont{Catani et~al.}(2009)\citenamefont{Catani, Cieri,
<   Ferrera, de~Florian, and Grazzini}}]{Catani:2009sm}
< \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Catani}},
<   \bibinfo{author}{\bibfnamefont{L.}~\bibnamefont{Cieri}},
<   \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Ferrera}},
<   \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{de~Florian}},
<   \bibnamefont{and} \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Grazzini}}
<   (\bibinfo{year}{2009}), \eprint{0903.2120}.
< 
541a491,517
> \bibitem[{\citenamefont{Ladinsky and Yuan}(1994)}]{Ladinsky:1993zn}
> \bibinfo{author}{\bibfnamefont{G.~A.} \bibnamefont{Ladinsky}} \bibnamefont{and}
>   \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
>   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D50}},
>   \bibinfo{pages}{4239} (\bibinfo{year}{1994}), \eprint{hep-ph/9311341}.
> 
> \bibitem[{\citenamefont{Balazs and Yuan}(1997)}]{Balazs:1997xd}
> \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Balazs}} \bibnamefont{and}
>   \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
>   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D56}},
>   \bibinfo{pages}{5558} (\bibinfo{year}{1997}), \eprint{hep-ph/9704258}.
> 
> \bibitem[{\citenamefont{Landry et~al.}(2003)\citenamefont{Landry, Brock,
>   Nadolsky, and Yuan}}]{Landry:2002ix}
> \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Landry}},
>   \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Brock}},
>   \bibinfo{author}{\bibfnamefont{P.~M.} \bibnamefont{Nadolsky}},
>   \bibnamefont{and} \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
>   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D67}},
>   \bibinfo{pages}{073016} (\bibinfo{year}{2003}), \eprint{hep-ph/0212159}.
> 
> \bibitem[{\citenamefont{Balazs and Yuan}(1999)}]{Balazs:1998bm}
> \bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Balazs}} \bibnamefont{and}
>   \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
>   \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D59}},
>   \bibinfo{pages}{114007} (\bibinfo{year}{1999}), \eprint{hep-ph/9810319}.
> 

